Exploiting Rich Syntax for Better Knowledge Base Question Answering

Recent studies on Knowledge Base Question Answering (KBQA) have shown great progress on this task via better question understanding. Previous works for encoding questions mainly focus on the word sequences, but seldom consider the information from syntactic trees.In this paper, we propose an approach to learn syntax-based representations for KBQA. First, we encode path-based syntax by considering the shortest dependency paths between keywords. Then, we propose two encoding strategies to mode the information of whole syntactic trees to obtain tree-based syntax. Finally, we combine both path-based and tree-based syntax representations for KBQA. We conduct extensive experiments on a widely used benchmark dataset and the experimental results show that our syntax-aware systems can make full use of syntax information in different settings and achieve state-of-the-art performance of KBQA.

==> coling2020/0_abstr.tex <==
\begin{abstract}
%In the research of knowledge base question answering(KBQA), the method based on semantic parsing can understand and analyze the question effectively, and  achieves good performance. In the previous researches, most of them were limited to word-level representation for questions. Obviously, this is not enough for the analysis of questions. Therefore, we use dependency syntax to obtain 
%more the semantic information of the question. Dependency syntax can not only structure a sentence to contain the structural information of the sentence, but also fully describe the dependency relationship between the words in the sentence. In this paper, as a supplement to character-level semantic encoding, we have tried a variety of dependency syntax encoding methods to semantically encode questions. And the experimental results on the baseline dataset show that combining dependency syntax helps to improve the system performance of KBQA.


Recent studies on Knowledge Base Question Answering (KBQA) have shown great progress on this task via better question understanding.
Previous works for encoding questions mainly focus on the word sequences, but seldom consider the information from syntactic trees.
In this paper, we propose an approach to learn syntax-based representations for KBQA. 
First, we encode path-based syntax by considering the shortest dependency paths between keywords. Then, we propose two encoding strategies 
to mode the information of whole syntactic trees to obtain tree-based syntax. Finally, we combine both path-based and tree-based syntax representations for KBQA.
We conduct extensive experiments on a widely used benchmark
dataset and the experimental results show that our syntax-aware systems can
make full use of syntax information in different settings and achieve state-of-the-art performance of KBQA.
    
\end{abstract}

% 基于知识库问答的研究中，基于语义解析的方法能够获取问句更多的信息，从而是模型性能会更好。但在之前的研究中，大部分都限于字符级别的语义解析，显然这样对于问句的解析是不够的。因而我们采用了依存句法来进行更深层次的挖掘出问句的语义信息。依存句法既可以将句子结构化使其包含句子的结构信息，也可以充分的描述句子中词与词之间的依存关系的依存句法。在本文中，作为对字符集语义编码的补充，我们分别尝试了多种依存句法的编码方法来对问句进行语义编码。并且在基线数据集上的实验结果表明，加入依存句法有助于提升KBQA的系统性能。


==> coling2020/1_intro.tex <==
\section{Introduction}
Question answering over knowledge base (KBQA) is an appealing task that arises with the advent of large-scale knowledge bases such as Freebase~\cite{bollackeretal:2008},  DBpedia~\cite{auer2007dbpedia}, and YAGO~\cite{suchaneketal:2007}. Briefly, this task is defined to be taking a natural language question as input and searching for an entity or an attribute value as an answer returned from knowledge bases. For example, the question ``{\em what movies did Diana play in?}" can be answered by translating the question into a triplet query {\em (Diana, play, ?)} that will be issued to a knowledge base. One key component of KBQA is question understanding which aims to transform a question into some semantic representation.

Approaches to question understanding can be broadly categorized into two groups. One group relies on the use of semantic parsing  techniques~\cite{Berant2013SemanticPO,reddy-etal-2014-large}. The main idea is to transform a natural language question into a formal meaning representation, eg., lambda calculus. The other group of approaches instead focus on generating query graphs directly with the aid of knowledge bases~\cite{Yih2015SemanticPV,Bao2016ConstraintBasedQA,Hu2018AnsweringNL,Luo2018KnowledgeBQ}.
Both solutions have gained a lot of attention, which are capable of obtaining plenty of essential question information.

%\Both solutions have gained a lot of attention which are capable of better question understanding

%\textcolor{red}{[to remove]Relatively, recent years have seen more interest in the latter group of approaches since semantic parsing approaches are apt to suffer from the limited sizes of datasets that are available for building the parsers.}

In recent years, the syntax information has also been investigated for better question understanding in KBQA since it is able to capture the connections between long distance words. One
representative approach is to use the shortest dependency path (SDP) from the answer word to an entity~\cite{Luo2018KnowledgeBQ}. This approach has brought remarkable results, since the path words are indeed important for understanding the questions.
% since the path words are indeed important for understanding the questions.
However, it mainly concerns the
connections between words, while neglects the representation of whole syntactic trees.  There exist tree-based syntax representations and it is interesting to examine whether incorporating richer syntactic information can further improve system performance. In this paper, we follow this direction and suggest to utilize dependency syntax to enhance the representation of questions in KBQA task. Dependency syntax is a widely used syntactic parsing formalism that captures interdependence between the words in a sentence, as illustrated in Figure~\ref{fig:dep_res}.

\begin{figure*}
  \centering
  \includegraphics[width=12cm]{coling2020/fig/dep_res.pdf}
  \caption{An example of dependency tree provided by the Stanford Parser.}
  \label{fig:dep_res}
\end{figure*}

In order to comprehensively explore the impact of syntactic information on KBQA performance, we propose to utilize three different methods to capture syntactic information, which are shortest dependency path (SDP), tree position feature (TPF), and Tree-GRU feature, respectively. The methods are designed from two different perspectives which consider path-based information and tree-based information respectively. Extensive experiments on a benchmark dataset show that the syntactic representations achieve significant improvements over the baseline system. By combining the syntax-based representations, we can further improve the performance of our systems. The contributions of the paper are as follows.

\begin{itemize}
%  \item For the first time, the entire tree of dependency syntax is used for encoding in the KBQA task. On one hand, we use the Tree-GRU neural network to encode the entire syntax tree. On the other hand, we also try combining the position information of each node to encode the entire syntax tree. The experimental results of the WebQuestion dataset also verify that the entire dependency syntax tree coding information has a positive improvement in the KBQA task.
%  \item \textcolor{red}{comprehensively analyzing the performance of the three mainstream coding methods(SDP, TPF, Tree-GRU) belonged to dependency syntax in the KBQA task. We carried out the respective coding experiments and mutual combination experiments according to the three methods.}

\item We experiment with two types of syntax-based representations, path-based and tree-based syntax representations to better encode the information of questions for KBQA. There are two methods
for modeling whole syntax trees to obtain tree-based representations. To the best of our knowledge, it is the first time that the information from entire syntax trees is used for KBQA.

\item We utilize the syntax-based representations for KBQA in different settings. The experimental results show that the proposed approach can effectively improve the performance of a state-of-the-art baseline system.

\end{itemize}



==> coling2020/3_approach.tex <==

\begin{figure*}
  \centering
  \includegraphics[width=16cm]{coling2020/fig/QA_encoding.pdf}
  \caption{The main structure diagram of our KBQA system. The methods and conditions in the dotted frame are not necessarily used.}
  \label{fig:querygraph}
\end{figure*}

%\section{Syntactic Parses Representation}
%\section{Approaches to Syntax Representation}
\section{Syntax-Aware Approach}
In this section, we describe three different  methods to encode syntactic information of a question from diverse perspectives. 
\begin{itemize}
  \item SDP (shortest dependency path) is the shortest path between the target word $w_{i}$ and the word $w_{a}$ that refers to the answer node in the parse tree. See details in Section~\ref{sdp_method}.
 \item TPF (tree position feature): For each word $w_{i}$ in a question, we compute the distance of the word to the root word $r_i$ in the parse tree. Such distance is regarded as a position feature. See details in Section~\ref{tpf_method}.
  \item Tree-GRU (tree-structured gated recurrent unit): After obtaining the dependency tree of a question, we encode the whole tree by using Tree-GRU and obtain a vector representation for each word $w_{i}$. See details in Section~\ref{tree_gru}.
\end{itemize}

As we can see, SDP is a path-based syntax representation, while TPF and Tree-GRU are tree-based representations that aim to capture global information of a parse tree. To incorporate syntactic information, we accumulate the encoding of dependency representations with the basic input $\bm{q}$ of each question. The architecture of our system is demonstrated in Figure~\ref{fig:querygraph}. 



\subsection{Path-Based Representation: SDP}
\label{sdp_method}
A shortest dependency path describes the path information of two specified words in a dependency  tree. %\textcolor{red}{Through the shortest dependency path, we can extract more meaningful words, to better model the dependency relationship between focus words.} 
Xu et al.~\shortcite{Xu2015ClassifyingRV} for the first time utilize neural network models to encode the shortest dependency path information between entities for the task of relation classification. For the task of KBQA, we can take the same approach for representing the dependencies between the focus words and the answer word, as illustrated in Figure~\ref{fig:sdp_dpl_tgru_tree} (a). The answer word usually starts with ``wh-" in a question, such as ``what" and ``who". The advantage of using shortest dependency paths as syntax representation is that it can capture salient information of the focus words to avoid interfering from non-important words. By using the shortest path method, the questions with multiple entities can be decomposed into several shortest dependent paths each of which corresponds to a focus word. 

Luo et al.~\shortcite{Luo2018KnowledgeBQ} apply the SDP method onto the KBQA task and have achieved remarkable improvements. Here, we adopt the same strategy. Specifically, given a question, we first recognize four types of focus words which are named entities, type words, time words, and ordinal words. We then collect a shortest dependency path for each focus word. Figure~\ref{fig:sdp_dpl_tgru_tree}(a) presents an illustrating example of a specific entity word, where the shortest dependency path corresponding to the word ``Diana" is ``what $\vec{det}$ movies $\vec{dobj}$ play $\vec{nsubj}$ Diana". To encode such a dependency path, we use pre-trained models like GloVe to initialize tokens in the path and then apply BiGRU to obtain the vector representation of the path. For focus words of other types, a similar process can be applied. For multiple different path representations, the maxpooling operation is used to extract the final vector. We finally get the encoding of the question using SDP, denoted as $\bm{x}_1^{syn}$.

\begin{figure*}
  \centering
  \includegraphics[width=15cm]{coling2020/fig/sdp_tpf_tgru_tree.pdf}
  \caption{Illustration of the encoding methods of SDP (a), TPF (b), and Tree-GRU (c).}
  \label{fig:sdp_dpl_tgru_tree}
\end{figure*}

\subsection{Tree-Based Representation: TPF}
\label{tpf_method}
Yang et al.~\shortcite{Yang2016APE} propose the tree position feature (TPF) for the task of relation classification, which could express the position information of each word in a dependency tree. Specifically, given a word $w_i$, we regard the root of a parse tree as a reference node and define the length of the path that connects the reference node and $w_i$ as the corresponding position feature. As shown in Figure \ref{fig:sdp_dpl_tgru_tree}(b), ``play" is the reference node, and the position feature of the word ``what" is $2$. Then, we convert the position features into  vectors by using random initialization.

In this way, for each word $w_i$ in a question, we can get its word embedding $\bm{w}_i$ and the corresponding tree position vector $\bm{d}_i$. Then we concatenate $\bm{w}_{i}$ and ${\bm{d}}_i$ to get the expression $\bm{z}_i=({{\bm{w}}_{i}},{\bm{d}}_i)$ for $w_i$. We apply BiGRU to encode the whole question and get the TPF-based representation, denoted as $\bm{x}_2^{syn}$. 


\subsection{Tree-Based Representation: Tree-GRU}
\label{tree_gru}
The approach to Tree-GRU based representation consists of two steps. The first step is pre-training on a large set of auto-parsed questions which learns the embeddings of dependency edges. The second step is the application of Tree-GRU to learn vector representations of the words in a question.

%\noindent \textbf{Pre-training of Edge Embeddings} 
%\\
\subsubsection{Pre-training of Edge Embeddings} 
We collect a set of 4.99M questions from multiple data sources, including SimpleQuestions ~\footnote{https://github.com/davidgolub/SimpleQA/tree/master/datasets/}, ComplexQuestions ~\footnote{https://github.com/JunweiBao/MulCQA/tree/}, Quora ~\footnote{https://www.kaggle.com/c/quora-insincere-questions-classification/data}$^,$~\footnote{https://www.kaggle.com/quora/question-pairs-dataset}, LC-QuAD 1.0~\footnote{http://lc-quad.sda.tech/lcquad1.0.html}, and LC-QuAD 2.0~\footnote{http://lc-quad.sda.tech/}. We then utilize the Stanford Parser to parse each question. %After processing, we will get the dependency syntax tree. For example, there is a center edge ``dobj" and its corresponding edge ``det" in the dependency syntax tree, as shown in Figure \ref{fig:sdp_dpl_tgru_tree}(c).
With the resulting set of auto-parsed questions, the skip-gram neural network language model~\cite{Mikolov2013EfficientEO} is used to pre-train embeddings of dependency edges. For an edge $a \xrightarrow{\textit{e}} b$ in a dependency tree, $a$ and $b$ are the head and tail of the edge $e$ respectively. Then we get the neighboring edges of the edge $a \xrightarrow{\textit{e}} b$ according to the dependency tree: 
$$\{ e_a\} \cup \{ e_b^1,e_b^2,\ldots, e_b^i,\ldots, e_b^n\},$$
where $\{ e_a\}$ represents the set of incoming edges of the node $a$ (except for the root node, each tree node has only one incoming edge), $\{e_b^i\}$ represents the set of outgoing edges of the node $b$, and $n$ refers to the number of outgoing edges of node $b$. The learning objective of skip-gram on the training data is to use the edge $a \xrightarrow{\textit{e}} b$ to predict neighboring edges . We finally obtain the pre-trained edge embeddings $\bm{E}_{e} \in \mathbb{R}^{|\bm{V}_e| \times d}$, where $|\bm{V}_e|$ denotes the number of all unique edges in auto-generated dependency trees and $d$ represents the dimension size of the pre-trained embeddings.

%\noindent \textbf{The Tree-GRU encoding} \\
\subsubsection{The Tree-GRU encoding}
Tree-GRU, as a variant of Tree-RNN, is an extension from sequence-structured GRU to tree-structured GRU~\cite{chen_etal_acl_2017}. Tree-GRU can learn global vector representations for each word in a question in a top-down and bottom-up learning process, as shown in Figure~\ref{fig:sdp_dpl_tgru_tree} (c). In the bottom-up learning process, the computation of $\bm{h}_{i}^\uparrow$ of each word $w_i$ is based on its child nodes. The detailed equations are as follows. 
%we use the bottom-up Tree-GRU encoding method. For each word in the question $W_i$ is encoded to get its semantic vector $h_i^\uparrow$, 

\begin{align}
&\bar{\bm{h}}_{i,L}^\uparrow = \sum_{j \in lchild(i)} \bm{h}_j^\uparrow ,  &\bar{\bm{h}}_{i,R}^\uparrow = \sum_{k \in rchild(i)} \bm{h}_k^\uparrow
\end{align}

\begin{equation*}
\begin{aligned}
& \bm{r}_{i,L}  =\sigma(\bm{W}^{rL}\bm{l}_{i}+\bm{U}^{rL} 
\bar{\bm{h}}_{i,L}^\uparrow +\bm{V}^{rL} 
\bar{\bm{h}}_{i,R}^\uparrow )\textrm{,} & \\
& \bm{r}_{i,R}  =\sigma(\bm{W}^{rR}\bm{l}_{i}+\bm{U}^{rR} 
\bar{\bm{h}}_{i,L}^\uparrow +\bm{V}^{rR} 
\bar{\bm{h}}_{i,R}^\uparrow )\textrm{,} & \\
& \bm{z}_{i,L}  =\sigma(\bm{W}^{zL}\bm{l}_{i}+\bm{U}^{zL} 
\bar{\bm{h}}_{i,L}^\uparrow +\bm{V}^{zL} 
\bar{\bm{h}}_{i,R}^\uparrow )\textrm{,} & \\
& \bm{z}_{i,R}  =\sigma(\bm{W}^{zR}\bm{l}_{i}+\bm{U}^{zR} 
\bar{\bm{h}}_{i,L}^\uparrow +\bm{V}^{zR} 
\bar{\bm{h}}_{i,R}^\uparrow )\textrm{,} & \\
& \bm{z}_{i} =\sigma(\bm{W}^{z}\bm{l}_{i}+\bm{U}^{z} 
\bar{\bm{h}}_{i,L}^\uparrow +\bm{V}^{z} 
\bar{\bm{h}}_{i,R}^\uparrow )\textrm{,} & \\
& \hat{\bm{h}}_{i}^\uparrow =\tanh(\bm{W}\bm{l}_{i}+\bm{U}(\bm{r}_{i,L} \odot \bar{\bm{h}}_{i,L}^\uparrow) + \bm{V}(\bm{r}_{i,R} \odot \bar{\bm{h}}_{i,R}^\uparrow))\textrm{,} & \\
& \bm{h}_{i}^\uparrow = \bm{z}_{i,L} \odot \bar{\bm{h}}_{i,L}^\uparrow+ \bm{z}_{i,R} \odot \bar{\bm{h}}_{i,R}^\uparrow + \bm{z}_{i} \odot \hat{\bm{h}}_{i}^\uparrow \textrm{,}&
\end{aligned}
\end{equation*}
where $lchild (i)$ and $rchild (i)$ refer to the set of left and right children of node $w_i$, $\bm{l}_{i}$ represents the dependency edge label between $w_i$ and its parent node, $\bm{W}$, $\bm{U}$ and $\bm{V}$ are trainable parameters of the model. 
In the same way, we can get the encoding vector $\bm{h}_i^\downarrow$ of each word in the question through the top-down encoding method. Finally, we concatenate the resulting hidden vectors obtained by these two encoding methods to get the final representation of a word:

\begin{align}
    \bm{t}_{i} &= \bm{h}_i^\uparrow \oplus \bm{h}_i^\downarrow
\end{align}
By concatenating the word embedding $\bm{w}_i$ and Tree-GRU embedding $\bm{t}_{i}$, we cat get the vector representation  $\bm{z}_i=\{\bm{w}_i,\bm{t}_{i}\}$ for the word $w_i$. We then apply BiGRU to obtain the Tree-GRU based representation of the question, denoted as $\bm{x}_3^{syn}$.

\subsection{Syntax-Aware System}
For a question, we have basic representation $\bm{q}$ (described in Section \ref{sec:basicencode}) and three types of syntax-based representations, $\bm{x}_1^{syn}$ (SDP), $\bm{x}_2^{syn}$ (TPF), and $\bm{x}_3^{syn}$ (Tree-GRU). Then, we directly accumulate these representations to obtain new representation of the question. Finally, we adopt the same training objective and optimization algorithm with the baseline.


==> coling2020/4_experiments.tex <==


\section{Experiments}
In this section, we evaluate the effect of different syntax-based representations for KBQA and conduct the experiments on a widely used dataset.

\subsection{Experimental Setup}
\subsubsection{Datasets}
We adopt the benchmark dataset WebQuestions~\cite{Berant2013SemanticPO}, which has been widely used in many recent works for the task of KBQA~\cite{Qu2018QuestionAO,Luo2018KnowledgeBQ}. The WebQuestions dataset contains both simple and complex questions, which are collected from Google Suggest API. We use the standard data split: 3,778 question-answer pairs for training and 2,032 pairs for testing. To tune the parameters of the systems, we randomly select about 20\% (755 pairs) from the training set as the development test. 

As for the knowledge base, we use the complete Freebase dump~\footnote{http://dwz.win/qRM or https://github.com/syxu828/QuestionAnsweringOverFB/} as the settings in~\newcite{Luo2018KnowledgeBQ}. The knowledge base contains 46M entities and 5,323 predicates, and we use Virtuoso-engine~\footnote{http://virtuoso.openlinksw.com/} to host the knowledge base. To parse questions, we use Stanford Parser V3.5.1~\footnote{https://nlp.stanford.edu/software/lex-parser.html}. To initialize word embeddings, we utilize GloVe word vectors~\cite{Pennington2014GloveGV} and word vectors from ELMo \cite{Peters2018DeepCW}.
% 我们训练系统、模型所用数据集是WebQuestions(WebQ)\cite{Berant2013SemanticPO}.WebQ 数据集是包含简单问题和复杂问题的综合性较强的数据集，同时也是被KBQA研究所广泛使用的数据集\cite{Qu2018QuestionAO}\cite{Luo2018KnowledgeBQ}。我们将数据集划分为3100用来训练，678用来做验证集，2032用来做测试集，其中每个问题都会产生对应的查询图进行候选。为了和baseline\cite{Luo2018KnowledgeBQ}保持一致，我们采用完整的freebase数据\footnote{http://dwz.win/qRM or https://github.com/syxu828/QuestionAnsweringOverFB/}用作知识库，里面包含了46M个实体和5323个谓词，采用 Virtuosoengine来构建知识库\footnote{http://virtuoso.openlinksw.com/}
\subsubsection{Hyperparameters}
We tune the hyperparameters of the baseline and our systems on the development set. We adopt the brute-force grid search to decide optimal hyperparameters. Specifically, the dimension of GloVe word vectors is set to 300 and the dimension of ELMo is set to 1,024. The Adam optimizer adopts a batch size of 32. The dropout rate is set to 0.1 when using the TPF method and the Tree-GRU method. We also use a dropout layer after the embedding layer.  In order to render the results reliable, we run each experiment three times by using different random seeds and report the average value as the final result.

\begin{table*}[tb]
\begin{minipage}[b]{77mm}
\begin{tabular}{p{5cm} l}
\hline
Question Representation & F1($\%$) \\
\hline
Baseline (QUE) & 52.33 \\
%sdp       & 49.87 \\
%tpf       & 51.86 \\
%tgru      & 50.94 \\

QUE+SDP   & 52.96 \\
QUE+TPF   & 52.58 \\
QUE+Tree-GRU   & 52.12 \\
QUE+SDP+TPF   & 53.27 \\
QUE+SDP+Tree-GRU   & 53.35 \\
\hline
Baseline (QUE)+ELMo & 52.83 \\
QUE+SDP+TPF+ELMo  & 53.59 \\
QUE+SDP+Tree-GRU+ELMo  & 53.63 \\
\hline
\end{tabular}
\caption{Main results.}
\label{tab:dep_baseline}
\end{minipage}
\begin{minipage}[b]{77mm}
\begin{tabular}{p{5cm} c}
\hline
Method & F1($\%$) \\
%\hline
\hline
\newcite{Dong2015QuestionAO} & 40.8 \\
\newcite{yaoetal:2015} & 44.3 \\
\newcite{bastetal:2015} & 49.4 \\
\newcite{berantetal:2015} & 49.7 \\
\newcite{Yih2015SemanticPV} & 52.5 \\
\newcite{Bao2016ConstraintBasedQA} & 53.3 \\
\newcite{jainetal:2016} & 55.6 \\
%\newcite{abujabaletal:2017} & 51.0 \\
\newcite{cuietal:2017} & 34.0 \\
\newcite{Luo2018KnowledgeBQ} & 52.7 \\
\newcite{chenetal:2019} & 51.8 \\
\midrule
Baseline (QUE) & 52.33 \\
QUE+SDP+Tree-GRU  & 53.35 \\
QUE+SDP+Tree-GRU+ELMo  & 53.63 \\
%\midrule
\hline
\end{tabular}
\caption{Comparison with previous works.}
\label{tab:results}
\end{minipage}
\end{table*}

\subsection{Main Results}
Here, we demonstrate the effect of syntax-based  representations. We compare the following systems in the experiments: (1) Baseline (QUE): in the baseline system, we use the word vectors of GloVe to initialize word embeddings of questions. (2) QUE+SDP: we add the information of short dependency path (SDP) to Baseline. (3) QUE+TPF: we add the information of tree position features (TPF) to Baseline. (4) QUE+Tree-GRU: we add the information provided by Tree-GRU to Baseline. (5) QUE+SDP+TPF: we add the information of tree position features (TPF) to QUE+SDP. (6) QUE+SDP+Tree-GRU: we add the information provided by Tree-GRU to QUE+SDP.

%Base Results

%In the experiment, we systematically explore the application of three different dependency syntax encoding in KBQA. Compared with the standard word sequence encoding method, the reasonable integration of syntactic encoding modules can improve the performance of KBQA. Table \ref{tab:dep_baseline} shows the relevant experimental results. It should be noted that the four different submodules we built differ only in the way questions are encoded, and the processing of other parts is completely the same. We use the standard word vector coding as our Baseline, which is called ``que", and it is used to represent questions simply from the perspective of sequence. Correspondingly, ``sdp", ``tpf", and ``tgru" are encoded from the path, position, and global information in the dependency syntax.

Table \ref{tab:dep_baseline} shows the results. From the table we can find that adding SDP and TPF solely yields an improvement of $0.63\%$ and $0.25\%$ F1 scores respectively, while adding Tree-GRU slightly underperforms than Baseline (QUE). Then, we further use the syntax-based representations together and show better performance. Finally, our best system (QUE+SDP+Tree-GRU) outperforms Baseline by an absolute improvement of $1.02\%$ F1 score. These facts indicate that the syntax-based representations are effective in improving the KBQA systems. 



%As can be seen, there is a steady upward trend from ``que" and ``que + sdp" to ``que + sdp + tpf" or ``que + sdp + treegru", which demonstrates the role of different syntactic coding modules in improving the baseline. It is worth noting that the application of ``sdp" module in KBQA was first proposed in \cite{Luo2018KnowledgeBQ}, which essentially extracts a main path in the dependency syntax tree. Furthermore, we achieve new improvements by combining ``tpf" and ``treegru" modules to model the location and global information in the dependency tree, respectively. 

%add ELMo 
To further improve our systems, we utilize vectors of ELMo for word representations of questions. The results are depicted in Table~\ref{tab:dep_baseline}. From the results we can see that using ELMo results in a stronger baseline with an improvement of $0.6\%$ F1 score. In addition, ELMo can further enhance our previous best system (QUE+SDP+Tree-GRU) by an improvement of $0.28\%$ F1 score. Our new best system (QUE+SDP+Tree-GRU+ELMo) achieves the final score of $53.63\%$ with an improvement of $1.3\%$ over Baseline. These facts indicate that our proposed syntax-based representations are complement with the pre-trained language models.
  
%In order to verify that the combined improvement of this module is stable, we continue to introduce ELMO word vector feature for the experiment. The results show that different syntax encoding modules are effective in improving the baseline, and the introduction of ELMO further improved the experimental performance to 1.3 points.

\subsection{Comparison with Previous Approaches}
Table~\ref{tab:results} shows the comparison of our systems with previous works. The results show that our Baseline is a strong system and our final system achieves the second best score in the table. In the work of~\newcite{jainetal:2016}, they use the relatively complex fact memory network which has better reasoning ability for complex questions. In future, we may use our proposed syntax-based representations in their system.



%After verifying the effectiveness of the syntactic coding module, we also compare the merged system with other SOTA systems. As can be seen from Table \ref{tab:results}, our results exceed most previous system results and are only slightly lower than Jain's. In contrast to Jain's approach, we use only the generic BiGRU network, rather than the relatively complex fact memory network. On the whole, the syntax encoding modules are reliable to improve the interrogative sequence only by using BiGRU. These modules can also be used in the fact memory network to achieve a more perfect performance.


% \subsection{Comparison of experimental results}
% First of all, we compare the experimental results on the test set after adding dependency syntax encoding to our baseline system. Table \ref{tab:dep_baseline} shows the difference in details. ``que" refers to the baseline system method which uses only the word sequence information encoding. ``que+sdp" refers to the model method of adding dependency syntax by the SDP method to basline. ``que+sdp+tgru” refers to the combination of the TreeGRU and the SDP methods for dependent syntax encoding, and then added to the baseline model method. ``Que + sdp + tgru + elmo" means the model method after combining the word vector representation of elmo on the basis of ``que + sdp + tgru". From the results, we can see that before the elmo word vector representation is added, the effect of dependency syntax on question encoding is obviously improved. After adding the well-presented elmo word vector representation, the dependency syntax still has a good effect on the question encoding. From these two points, it can be proved that the dependency syntax does indeed improve the question expression on the KBQA task.

% In addition, from the results in Table 2, the performance of our best system ranked second in the list, which proves that our bset system has reached the state-of-the-art performance on the task. But compared with \cite{jainetal:2016}, ours is still slightly insufficient. So we first try to improve the performance of the dependency parser, which could improve the overall performance of the system. Finally, we Will also try to add dependent syntax encoding on \cite{jainetal:2016} to get better system performance.
%首先我们比较了在数据集上关于将依存句法编码加入我们的baseline系统之后的实验效果,"que"指的就是baseline系统方法即仅仅使用问句的词序列信息编码。“que+sdp”指的就是以sdp方法编码的依存句法加入到basline的模型方法。“que+sdp+tgru”指的就是结合了tgru和sdp方法进行依存句法编码，然后加入到baseline的模型方法。“que+sdp+tgru+elmo”表示是在“que+sdp+tgru”的基础上结合elmo的词向量表示后的模型方法。从结果我们可以看出，在没加入elmo词向量表示之前，依存句法对于问句编码的效果提升很明显。在加入了表现不错的elmo词向量表示后，依存句法依然对问句编码有不错的效果。从这两点就能证明依存句法对于KBQA任务上面的问句表示的确有不错的提升。

% 除此之外，从表2上的结果来看，我们的最好的性能上排到了第二名。但是和Jain的系统相比还有提升空间，因此我们首先会在依存句法的分析器上面进行系统的整体提升，另外还会再Jain的系统上尝试加入依存句法的编码来获得更好的系统性能。

\subsection{Analysis and Discussions}

% \begin{figure*}
%     \centering
%     \includegraphics[width=20cm]{coling2020/fig/question_length_F1.pdf}
%     \caption{The performance of baseline and syntax system in various length of question.}
%     \label{fig:length_f1}
% \end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=15.5cm]{coling2020/fig/ErrorAnalysis.pdf}
    \caption{Performance comparison of baseline and syntax-aware system.}
    \label{fig:analysis}
\end{figure*}


% \begin{figure*}
%     \centering
%     \includegraphics[height = 5cm,width=16cm]{coling2020/fig/question_type_F1.pdf}
%     \caption{The performance of baseline and syntax system in various question types.}
%     \label{fig:type_f1}
% \end{figure*}
We further compare the performance between Baseline and our system (QUE+SDP+Tree-GRU) to analyze the effect of syntactic information on question types and question lengths.

The results on question types are shown in Figure \ref{fig:analysis}(a). From the figure, we find that the syntax-aware system provides better performance on five types, while two systems yield similar scores for type ``\emph{which}". This indicates that the syntax-based representations can provide useful information for the general cases. 

%Among all the types, the syntax-based system achieves the largest improvement on ``\emph{how}". In type ``\emph{how}", there [some examples? or case study]

%We have experimented with three ways of introducing syntax into knowledge base question answering. Compared with the baseline method, the syntax method improve the matching performance between the question and the query graph. In order to explore the specific role of syntax, we compare the differences between baseline and the approach of fusing syntactic information. On the one hand, we compare the performance differences between the two methods according to the length of the question, the above of figure \ref{fig:analysis} shows the result. On the other hand we calculate the performance of different methods on different types of questions as the below of figure \ref{fig:analysis}.

The results on question lengths are shown in Figure \ref{fig:analysis}(b). we split the test set into three sets by the question length: SHORT(3-4), MID(5-7), and LONG(8+). From the figure,
we find that the improvement gap is larger on the LONG set than that on the MID and SHORT sets. The reason might be that the dependency trees can provide useful connections for the words with long distance.
%Through the performance of the two methods in different question lengths, we can see that the introduction of syntax can better answer the longer questions. We also find that the performance of the system decrease in the very short questions. We hold that it may be not necessary to introduce syntactic information in the very short questions, and the sequence coding is sufficient for thees short questions. Besides, from the comparison between the baseline system and the syntactic system, we can also
%find that the introduction of syntax can improve the performance of all types of questions, which indicates that syntax plays a universal role in all types of questions.

\begin{figure*}
    \centering
    \includegraphics[width=8cm]{coling2020/fig/case_tree.pdf}
    \caption{Case study: dependency tree of a question.}
    \label{case_tree}
\end{figure*}


\subsection{Case Study}
In this section, we check the results in more detail. We find that the syntax information is helpful for the cases where the constraint words are far away from the predicate words. Figure \ref{case_tree} shows the dependency tree of a real example for case study, where the question is ``What TV shows did Shawnee Smith play in?", in which ``TV shows" is the constraint words and ``play" is the predicate word. The baseline system can not identify the connection between ``TV shows" and ``play", while the syntax-aware system can have this information as shown in Figure \ref{case_tree}. Due to the lack of sufficient information, the baseline system  returns the wrong relationships ``film.actor.film" and ``film.performance.film", and fails to predict the correct answer. In contrast, the syntax-aware system can map to the correct relationships ``tv.tv\_actor.starring\_roles" and ``tv.regular\_tv\_appearance.series", and obtain the correct answer.



==> coling2020/5_relation_work.tex <==
\section{Related Work}

In the field of KBQA, there are two group of representative approaches: systems based on query graph generation and systems based on semantic parsing. The main idea of the former group is to apply information extraction techniques to construct structured queries which can be issued to knowledge bases to get the answer. A bunch of previous works have been conducted in this direction, includeing~\newcite{yaoetal:2014},~\newcite{Bordes2015LargescaleSQ},~\newcite{Dong2015QuestionAO},~\newcite{Bao2016ConstraintBasedQA},~\newcite{Xu2016QuestionAO},~\newcite{Hu2018AnsweringNL}, and~\newcite{Luo2018KnowledgeBQ}. The main difference between the approaches is the representation of query graphs. In contrast, the latter group of systems relies on semantic parsing techniques which often suffer from the lack of training data for build semantic parsers. The output of semantic parsing are queries in the form of formal meaning representation.~\newcite{Berant2013SemanticPO} and \newcite{Kwiatkowski2013ScalingSP} have proposed different models for semantic parsing of natural language questions. Our work focuses on incorporating rich syntax into a system that is built on query graph generation.


==> coling2020/6_conclusion.tex <==
\section{Conclusion}
In this paper, we show that utilizing the syntax-based representations can have a substantial effect on the performance of KBQA. In particular, we demonstrate that our systems consistently outperform a strong baseline system using ELMo. In our approach, we consider two types of 
syntax-based representations, path-based and tree-based representations. As for the tree-based representations, we model the whole syntactic trees to obtain global information. Furthermore, the experimental results show that two types of representations are complementary to each other in our final system.


%In this paper, we utilized three different dependency syntax representations to boost a KBQA system, including shortest dependency path, tree position feature, and Tree-GRU. Separately using the three different dependency syntax information and word sequences to improve the semantic interpretation of question sentences. The experimental results prove that, even if the stronger ELMO external word vector is used to enhance the model, dependency syntax can still achieve good performance in KBQA. Similarly, by using ELMO and dependency syntax coding, our final model has achieved good results on the WebQ dataset. %Since the syntactic analyzer we use is the Stanford syntactic parser \footnote{https://nlp.stanford.edu/software/lex-parser.shtml\#Download}, although it is classic, there are still some deviations. These deviations indicate that there is still probability for further improvement in the parsing of the dependency syntax tree. In the future, we may try to use more precise dependency syntax analysis to improve the effect of dependency syntax, which can further improve the performance of KBQA.



